Rethinking Translation Memory Augmented Neural Machine Translation

This paper rethinks translation memory augmented neural machine translation (TM-augmented NMT) from two perspectives, i.e., a probabilistic view of retrieval and the variance-bias decomposition principle. The finding demonstrates that TM-augmented NMT is good at the ability of fitting data (i.e., lower bias) but is more sensitive to the fluctuations in the training data (i.e., higher variance), which provides an explanation to a recently reported contradictory phenomenon on the same translation task: TM-augmented NMT substantially advances vanilla NMT under the high-resource scenario whereas it fails under the low-resource scenario. Then we propose a simple yet effective TM-augmented NMT model to promote the variance and address the contradictory phenomenon. Extensive experiments show that the proposed TM-augmented NMT achieves consistent gains over both conventional NMT and existing TM-augmented NMT under two variance-preferable (low-resource and plug-and-play) scenarios as well as the high-resource scenario.

==> 1-intro-bak.tex <==
\section{Introduction}
\label{section:introduction}

The effectiveness of Translation Memory (TM) in the task of Neural Machine Translation (NMT) has long been recognized, and many notable approaches have been proposed to augment NMT models by using a TM \citep{feng-etal-2017-memory,gu2018search,DBLP:conf/ecai/CaoKX20,he-etal-2021-fast,cai-etal-2021-neural,2105.13072}. 
A TM is originally collected from the translation history of professional translators, and provides the most similar source-target sentence pairs for the source sentence to be translated \citep{garcia2009beyond, koehn2010convergence, utiyama2011searching, he-etal-2021-fast}.

Although a TM generally provides valuable translation information particularly for those input sentences preferably matching the source sentences of the TM in both statistical machine translation models \citep{wang2013integrating, liu2019unified} and neural machine translation models \citep{gu2018search, cai-etal-2021-neural, he-etal-2021-fast}, it may cause performance degradation if the size of TM datastore is small and thus the retrieved TM is less relevant with current sentence to be translated \citep{hoang2022improve_Robustness_TM_NMT}, and in this scenario, the generalization ability of models plays an important role. 

Recently, \citet{cai-etal-2021-neural} find that in the low resource scenario (i.e. the training pairs are very scarce), a small size of TM datastore even hurts the model performance compared with vanilla Transformer, and they use monolingual translation memory to solve the problem of insufficient training data.
However, it is unclear how the number of TMs influence the generalization ability of models qualitatively and quantitatively because TMs introduce more variables which NMT models condition on.


\begin{table}[t]
\centering
\begin{tabular}{c|c|c}
\hline
\textbf{Model} & \textbf{Full} & \textbf{Quarter} \\
\hline
\makecell[c]{vanilla \\ Transformer} &  60.83  & 54.54   \\
\hline
\makecell[c]{TM augmented \\ NMT} &  63.76  & 53.92   \\
\hline
\end{tabular}
\caption{Test BLEU and perplexity of vanilla Transformer and TM augmented NMT models with full train data and quarter train data respectively.}
\label{table:preliminary}
\end{table}


In order to measure the influence brought by the generalization ability of TM augmented NMT models quantitatively, we conduct a preliminary experiment on the JRC-Acquis German $\Rightarrow$ English (De $\Rightarrow$ En) dataset. 
We use full train data and quarter train data to train a vanilla Transformer \citep{vaswani2017attention} and a TM augmented NMT model with top-5 TMs \footnote{Note that this backbone is used in \citet{cai-etal-2021-neural} and it is a strong baseline.} respectively. 
It is well known that the generalization ability of a model can be reduced as the amount of training data decreases\citep{niyogi1996generalization, bishop2006pattern}, then we observe the difference of performance brought by the different generalization abilities of TM augmented NMT models and compare them with vanilla Transformer\citep{vaswani2017attention}. Table \ref{table:preliminary} shows BLEU and perplexity of these models on test dataset. The detailed settings for this experiment are shown in Appendix ~\ref{appendix_sec:preliminary}.

In Table \ref{table:preliminary}, TM augmented NMT model is better than vanilla Transformer if trained with full data. 
However, when models are trained with quarter data, performance of TM augmented NMT model is degraded more compared with that of vanilla Transformer. 
According to this phenomenon, we hypothesize tentatively that the generalization ability of TM augmented NMT models is lower than that of vanilla Transformer in this low scenario, which motivates us to study some methods to alleviate the negative impact of low generalization ability in TM augmented NMT models.

In this paper, we verify the hypothesis about low generalization ability of TM augmented NMT model from bias-variance perspective, then propose a series of methods to promote the generalization ability of TM augmented NMT model. 
We firstly change the top-5 TMs as in \citet{Xia_Huang_Liu_Shi_2019} and \citet{cai-etal-2021-neural} to top-1 TM according to our results of bias-variance decomposition. 
We find that the size $K$ is a trade-off between variance and bias. That is to say, when $K$ is set to be 1, the variance of TM augmented model is the smallest while the bias is also the largest, especially under the low resource scenario. As $K$ increases, more TMs reduce bias while bring more variance meanwhile.
Then, we intuitively use average ensemble of top-5 TMs to retain the generalization ability of top-1 TM method and get more useful information from top-5 TMs meanwhile. 
Finally, we propose a lightweight network to weighted ensemble top-5 TMs. 
To validate the effectiveness of the proposed approach, we conduct extensive experiments on several translation tasks under different scenarios including low resource scenario, plug and play scenario and general translation scenario.

Contributions of our method are three folds:
\begin{itemize}
    \item We rethink and analyse the generalization ability of translation memory augmented neural machine translation models from bias-variance decomposition perspective.
    \item We propose a simple yet effective lightweight network to ensemble translation memory augmented neural machine translation models, whose variance is small and bias is also relatively small.
    \item Our experiments prove the effectiveness of the aforementioned approach, it outperforms both vanilla Transformer and baseline translation memory augmented neural machine translation models under low resource scenario, plug and play scenario, and conventional machine translation scenario.
\end{itemize}



==> 4-method-bak.tex <==
\section{Proposed Approach for Lower Variance}
\label{section:proposed_approach}
In this section, we first propose two techniques to reduce the variance of the TM augmented NMT model. Then we propose a new TM-augmented NMT on the basis of the two techniques to address the contradiction phenomenon as presented in Section.  
Finally we empirically quantify the variance and bias for the proposed TM-augmented NMT. Note that the proposed TM-augmented NMT is general to be applied on top of any specific TM augmented NMT models. 


\subsection{Conditioning on One TM Sentence}
\label{subsection:change_number_of_TMs}
In conventional TM augmented NMT, the translation model $P(\mathbf{y}|\mathbf{x}, \mathbf{Z})$ is conditioned on $\mathbf{Z}$ consisting of five retrieved TMs $\{\mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5\}$ with $\mathbf{z}_i = ( \mathbf{x}_i^\text{tm}, \mathbf{y}_i^\text{tm} )$. 
Similar to the analysis in Eq.(\ref{eq:lvm}-\ref{eq:TM-lvm}), we can obtain the following equations:
\begin{equation*}
\begin{aligned}
    P(\mathbf{y}|\mathbf{x}, \mathbf{z}_1) = & \sum_{\mathbf{z}_2, \cdots, \mathbf{z}_5} P(\mathbf{y}|\mathbf{x}, \mathbf{z}_1, \mathbf{Z}_{>1}) P(\mathbf{Z}_{>1}|\mathbf{x}, \mathbf{z}_1)  \\
  = & \sum_{\mathbf{z}_2, \cdots, \mathbf{z}_5} P(\mathbf{y}|\mathbf{x}, \mathbf{z}_1, \mathbf{Z}_{>1}) P(\mathbf{Z}_{>1}|\mathbf{x})   \\
  \approx & P(\mathbf{y}|\mathbf{x}, \mathbf{Z}), \text{  with  } \mathbf{Z}_{>1} \sim P(\mathbf{Z}_{>1}|\mathbf{x}). 
\end{aligned}
\end{equation*}
\noindent where $\mathbf{Z}_{>1}=\{\mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5\}$, and the second equation holds due to the conditional independence assumption in Eq.~\eqref{eq:cd}. In this sense, we can see that $P(\mathbf{y}|\mathbf{x}, \mathbf{Z})$ conditioned on five retrieved TMs is actually an approximation of $P(\mathbf{y}|\mathbf{x}, \mathbf{z}_1)$ conditioned on a single retrieved TM $\mathbf{z}_1$.  As a result, as analysed in Section 2.1, whether $P(\mathbf{y}|\mathbf{x}, \mathbf{Z})$ is a good estimator depends on the variance with respect to $\mathbf{Z}_{>1}$, i.e., $\mathbb{V}_{\mathbf{Z}_{>1}} P(\mathbf{y}|\mathbf{x}, \mathbf{z}_1, \mathbf{Z}_{>1})$.

% From the analysis in \S\ref{subsection:view_from_latent_variable_model}, we can get the relationship theoretically between the variance related to $\mathbf{z}_1$ and that related to $\{\mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5\}$ as follows:

% \begin{multline}
%   \mathbb{V}_{\mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5} P(\mathbf{y} | \mathbf{x}, \mathbf{z}_1, \mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5)  \\
%   > \mathbb{V}_{\mathbf{z}_{1}} P(\mathbf{y} | \mathbf{x}, \mathbf{z}_1) 
% \end{multline}
% \noindent where the left side stands for the variance using 5 TMs and the right side is the variance with only one TM.

% It is also intuitive since the extra four TMs ${\mathbf{z}_2, \mathbf{z}_3, \mathbf{z}_4, \mathbf{z}_5}$ are extra variables compared with the model with one TM, and hence the variance is higher. Therefore, it is reasonable to use only one TM in TM augmented NMT models since it has lower variance.

Based on the above analysis, to alleviate the variance, we directly estimate $P(\mathbf{y}|\mathbf{x})$ by using a single sampled sentence pair. Formally, 
suppose $\mathbf{z}=\langle \mathbf{x}^\text{tm}, \mathbf{y}^\text{tm} \rangle $ is a {\bf single} bilingual sentence sampled from $P(\mathbf{z}|\mathbf{x})$, we apdot the following TM-augmented NMT conditioned on a single retrieved sentence $\mathbf{z}$:
\begin{equation}
\small
\label{eq:tm-cond-one}
\begin{aligned}
    & P(y_t | \mathbf{x}, \mathbf{y}_{<t})=\mathbb{E}_z P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}) \approx P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}) ,\\
    & P(\mathbf{y}|\mathbf{x})=\prod_{t} P(y_t | \mathbf{x}, \mathbf{y}_{<t}) \approx \prod_{t} P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}) , \\
\end{aligned}
\end{equation}
\noindent where $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z})$ can be any model architecture of TM-augmented NMT models $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{Z})$ by replacing top-$K$ TMs $\mathbf{Z}$ with a single top-1 TM $\mathbf{z}$. In addition, the training of the above model $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z})$ is the same as the training of the conventional model $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{Z})$.

\subsection{Average Ensemble}
\label{subsection:average_ensemble}
In Equation~\eqref{eq:tm-cond-one}, $\mathbb{E}_z P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z})$ is approximated by one sample $\mathbf{z}$, which still induces some potential estimation errors due to the variance $\mathbb{V}_\mathbf{z} P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z})$. In fact, the estimation errors can be further reduced by the estimation using multiple samples according to the following Lemma.
\begin{lemma}
If $\mathbf{z}_1, \cdots, \mathbf{z}_K$ are independent and identically distributed random variables sampled from the $P(\mathbf{z}|\mathbf{x})$, then the following inequality holds:
\begin{multline*}
    \mathbb{V}_{\mathbf{z}} P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}) \ge \\ \mathbb{V}_{\mathbf{z}_1, \cdots, \mathbf{z}_K} \Big(\frac{1}{K}\sum_k P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_k)\Big)
\end{multline*}
\end{lemma}
\noindent The proof of this Lemma is presented in the appendix~\ref{xx}. 

% In previous discussions, we analyse the variance from the theoretical and experimental point of view in sentence level. Since neural machine translation is a sequence to sequence task with auto regressive manner, we can further breakdown the probabilistic model defined by Eq.~\eqref{eq:TM-lvm} to a more fine-grained form in token level as follows:

% From Lemma ~\ref{lemma:variance_of_latent_variable_model}, we can draw two conclusions: 
% (1) With the sample size $s$ increasing, the variance of right side of the inequality in Lemma ~\ref{lemma:variance_of_latent_variable_model} will decrease obviously because the denominator of that becomes larger.
% (2) Since the introduction of the variable $\mathbf{Z}^{1}, \cdots, \mathbf{Z}^{s}$, the variance of right side of the inequality in Lemma ~\ref{lemma:variance_of_latent_variable_model} related to variables $\mathbf{Z}^{1}, \cdots, \mathbf{Z}^{s}$ is larger than that of $P(\mathbf{y} | \mathbf{x})$ related to $\mathbf{Z}^{1}, \cdots, \mathbf{Z}^{s}$. In the extreme case when the sample size $s$ goes to infinity, that variance goes to zero meanwhile, which is the same as the variance of $P(\mathbf{y} | \mathbf{x})$ related to $\mathbf{Z}^{1}, \cdots, \mathbf{Z}^{s}$.

According to the above Lemma, we propose the method to approximate $P(y_t|\mathbf{x}, \mathbf{y}_{<t})$ through the average ensemble of all $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_k)$:
\begin{equation}
\label{eq:tm-sum-k}
\begin{aligned}
& P(y_t | \mathbf{x}, \mathbf{y}_{<t}) \approx \frac{1}{K}\sum_i P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}) \\
    & P(\mathbf{y}|\mathbf{x})  \approx  \prod_{t=1}^m \sum\limits_{k=1}^{K} P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k}).
\end{aligned}
\end{equation}
Note that we do not particularly retrain the averaged ensemble model by directly taking the parameters from the model $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z})$ trained in \S4.1 in this paper.
% Therefore, we directly apply the average ensemble top-5 TMs method to the trained model in \S~\ref{subsection:change_number_of_TMs} and compute the variance-bias decomposition results, which are shown in the fifth column of Table ~\ref{table:variance_all_models}.


\paragraph{Remark} The above average ensemble model involves $K$ retrieved sentence pairs similar to the standard translation memory augmented models~\cite{gu2018search,zhang-etal-2018-guiding,cai-etal-2021-neural}, but the notable difference is that our model $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k})$ conditions on a single $\mathbf{z}_{i}$ whereas those standard NMT models (see Equation~\eqref{equation:TM-nmt-original}) directly condition on $K$ retrieved sentence pairs $\mathbf{Z}=\{\mathbf{z}_k\}_{k=1}^K$.  

% It can be easily deduced that the average ensemble method is just setting $w(\mathbf{x}, \mathbf{y}_{<t}, Z^{i})$ to $\frac{1}{s}$.

\subsection{Weighted Ensemble}
In our experiments as shown in \S\ref{subsection:empirical_analysis_variance} later, we found that the average ensemble delivers better variance but sacrifices its ability of fitting data (i.e., bias) compared to the standard TM-augmented NMT conditioning on all retrieved $\mathbf{Z}=\{\mathbf{z}_k\}_{k=1}^K$.  
In order to further improve our average ensemble method, we propose the weighted ensemble to establish a stronger relationship between the source sentence and each TM $\mathbf{z}_k$ by endowing more powerful representation ability via the weighting coefficient $w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}^{i})$ in Eq.~\eqref{equation:TM-nmt-latend_variable_token_level}. Formally, the weighted ensemble model is defined as:
\begin{equation}
\label{equation:TM-nmt-latend_variable_token_level}
\begin{aligned}
    P(\mathbf{y}|\mathbf{x})  \approx  \prod_{t=1}^m \sum\limits_{k=1}^{K} w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k}) P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k}),
\end{aligned}
\end{equation}
\noindent where $P(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k})$ can be any TM-augmented model architecture as claimed in \S\ref{subsection:change_number_of_TMs}, and $w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k})$ is a weighting network via the following equation:
 % \begin{equation}
 % \label{equation:w}
 %     w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{i}) = \text{Softmax}(\text{FFN}(H_t, \sum\limits_{i=1}^{K} \frac{c_{t,i}}{K}))
 % \end{equation}
\begin{equation}
\label{equation:w_k_in_TMNMT}
    w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k}) = \text{Softmax}\big(f(H_t, {H_{t,k}})\big)[k],
\end{equation}
\noindent where $f$ consists of two linear layers with residual connection and layer normalization \citep{vaswani2017attention}, $H_t$ is the decoding state of a vanilla translation model $P(y_t|\mathbf{x}, \mathbf{y}_{<t})$, $H_{t,k}$ is the decoding state for any TM-augmented model $P(y_t|\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_k)$ similar to $H_{t,\mathbf{Z}}$ in Eq.~\eqref{eq:equation:TM-nmt-original}. 
For example, if we implement the weighted ensemble model on top of the model architecture of \citet{cai-etal-2021-neural}, then the source sentence and the $k$-th TM are encoded by two separate encoders respectively, resulting in a hidden state $H_t$ for current time step and a contextualized TM representation $H_{t,k}$ for the $k$-th TM in current time step. 

% After we get each $P_{k}(y_t | \mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{i})$ for each TM, finally, we use the proposed lightweight network to compute weights for weighted ensemble $w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}^{k})$. The lightweight network is defined as follows:

Similar to average ensemble method, we do not train the whole network from scratch. Instead, we start from the trained model parameters of $P(y_t|\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_k)$ in \S\ref{subsection:change_number_of_TMs} and then we just fine-tune the whole parameters including those from both $P(y_t|\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_k)$ and $w(\mathbf{x}, \mathbf{y}_{<t}, \mathbf{z}_{k})$ for only about 2,000 updates on $90\%$ part of valid data while the other $10\%$ part of valid data are used to select the checkpoint for testing.

%\begin{table}[t]
%\setlength{\tabcolsep}{1.5pt}
%% \scriptsize
%\renewcommand\arraystretch{2}
%\centering
%\begin{tabular}{|m{2.5cm}<{\centering}|m{2cm}<{\centering}m{2cm}<{\centering}|}
%% \toprule
%\hline
%{\textbf{Model}} & {\textbf{Var}} & {\textbf{$\text{Bias}^2$}} \\
%\hline
%{w/o TM}  & 0.1573 &  1.9992 \\
%\hline
%{TM-base} & 0.2168 & \textbf{1.8460} \\
%\hline
%{TM-single} & 0.1944 &  1.9369  \\
%\hline
%{TM-average} & 0.1918  & 1.9395   \\
%\hline
%{TM-weight} & \textbf{0.1814} & 1.9137 \\
%\hline
%\end{tabular}
%\caption{Estimated variance and bias. w/o TM denotes the NMT model without TM, TM-base denotes the default TM-augmented NMT conditioned on five TMs; and TM-single, TM-average, and TM-weight are three models proposed in \S4.}
%\label{table:variance_all_models}
%\end{table}

\begin{table}[t]
%\setlength{\tabcolsep}{1.5pt}
%\scriptsize
\small
\renewcommand\arraystretch{2}
\centering
\begin{tabular}{m{0.8cm}<{\centering}|m{1cm}<{\centering}|m{0.8cm}<{\centering}|m{0.8cm}<{\centering}|m{0.8cm}<{\centering}|m{0.8cm}<{\centering}}
% \toprule
\hline
{\textbf{Model}} &  \makecell[c]{w/o TM} & {TM-base} &  {TM-single} & {TM-average} & {TM-weight} \\
\hline
{\textbf{Var}} &  0.1573 & 0.2168 & 0.1944  &  0.1918  & \textbf{0.1814} \\
\hline
{\textbf{$\text{Bias}^2$}} &  1.9992 & \textbf{1.8460} & 1.9369  &  1.9395  & 1.9137 \\
 %\bottomrule
\hline
\end{tabular}
\caption{Estimated variance and bias. w/o TM denotes the NMT model without TM, TM-base denotes the default TM-augmented NMT conditioned on five TMs; and TM-single, TM-average, and TM-weight are three models proposed in \S\ref{section:proposed_approach}.}
\label{table:variance_all_models}
\end{table}

\subsection{Empirical Analysis on Bias and Variance}
\label{subsection:empirical_analysis_variance}
\lm{Please improve this subsection.}

In order to verify the effectiveness of three proposed methods empirically, we conduct the variance-bias decomposition experiments similar to \S\ref{subsection:bias_variance_decomposition} and do empirical analysis. 
Specifically, we estimate variance and bias of both three proposed models and two baselines including vanilla Transformer without TM \citep{vaswani2017attention} and default TM-augmented NMT conditioned on five TMs. 
We implement our proposed methods on top of the dual encoder architecture of \citet{cai-etal-2021-neural} without loss of generality since our methods can be applied to any specific TM augmented NMT models.

Table ~\ref{table:variance_all_models} shows the overall results of estimated variance and bias.
By comparing results of different models, we can get the following two observations:
Firstly, through the results of variance, we can find that three proposed methods all achieve lower variance compared with the default TM-augmented NMT model. And it is notable that the weighted ensemble method achieves the best variance within all the TM-augmented NMT models.
Secondly, through the results of bias, we can find that all TM-augmented NMT models achieve lower bias compared with vanilla Transformer\citep{vaswani2017attention} without TM. Although our methods have slightly higher bias, the proposed weighted ensemble method can achieve comparable bias with regard to the default TM-augmented NMT model.

In conclusion, through rigorous theoretical derivation and reasonable experimental design, we can get a glimpse of the proposed methods especially weighted ensemble's potential advantages by bias-variance decomposition theoretically and empirically.


